Optimal Sensing of Momentum Kicks with a Feedback-Controlled Nanomechanical Resonator

External disturbances exciting a mechanical resonator can be exploited to gain information on the environment. Many of these interactions manifest as momentum kicks, such as the recoil of residual gas, radioactive decay, or even hypothetical interactions with dark matter. These disturbances are often rare enough that they can be resolved as singular events rather than cumulated as force noise. While high-Q resonators with low masses are particularly sensitive to such momentum kicks, they will strongly excite the resonator, leading to nonlinear effects that deteriorate the sensing performance. Hence, this paper utilizes optimal estimation methods to extract individual momentum kicks from measured stochastic trajectories of a mechanical resonator kept in the linear regime through feedback control. The developed scheme is illustrated and tested experimentally using a pre-stressed SiN trampoline resonator. Apart from enhancing a wide range of sensing scenarios mentioned above, our results indicate the feasibility of novel single-molecule mass spectrometry approaches.

==> ExperimentalSetup.tex <==
\section{Filter and Controller Implementation} \label{sec:experimental_setup}
%To validate the algorithms presented in the previous section, we conduct experiments on an apparatus tailored for ultra-sensitive force detection. We employ a high-Q prestressed silicon nitride trampoline resonator for this purpose. The selected resonator boasts a thickness of \SI{50}{nm}, a frame edge length of \SI{1}{mm}, a tether width of $5$\textmu\SI{}{\meter}, and a central pad measuring 45\textmu m by 45\textmu m. Actuation is facilitated by two gold wires, each with a thickness of \SI{200}{nm} and a width of $2.5$\textmu\SI{}{\meter}, coated onto the tethers. The resonator is immersed in a magnetic field of $\thicksim 1$T originating from two neodymium magnets located to the sides of the resonator. Thus the wires enabled the application of Lorenz forces upon the resonator when a current was passed through them. To mitigate gas damping from the surroundings, the resonator was situated within an high vacuum (HV) chamber, maintaining a residual pressure of $<$ \SI{1e-5}{mbar}.
%
%For measurements, a commercial laser Doppler vibrometer with a laser wavelength of \SI{638}{nm}, operating in a heterodyne regime, was employed. The data captured by the vibrometer's photo diode was recorded and processed using a RedPitaya field programmable gate array (FPGA) board before being transmitted to a laboratory computer. Additionally, to apply force to the resonator, the output of the FPGA was connected to the resonator's actuated wires via a Digital-Analog Converter. Figure (\ref{fig:expSetup1}) illustrates the experimental setup.
%
%The Q-factors of the resonators modes were determined through ring-down measurements, yielding values on the order of $10^5$, with resonance frequencys on the order of tens of kilohertz. To validate these findings, they were compared against results obtained from finite element analysis conducted with COMSOL. Table (\ref{tab:NEMSModes}) presents a comparison of experimental and simulated system parameters. As expected, only modes predominantly oscillating out of plane significantly contributed to the oscillating effective mass of the resonator. This observation is evident in figure (\ref{fig:ResSpec}), which depicts the measured and theoretical spectra of the oscillator between 0 and \SI{180}{kHz}. Prominent peaks are observed at \SI{23}{kHz}, \SI{68}{kHz}, and \SI{114}{kHz}, aligning with corresponding mode shapes and frequencies from simulations. Additionally, parasitic peaks at \SI{21}{kHz} and \SI{42}{kHz} are evident, likely originating from unknown oscillation processes in the measurement apparatus, as they persist in measurements without a resonator. Furthermore it can be seen, that the detection noise floor is colored meaning, that it increases over the frequency range of the measurement.
%
%\subsection{Filter and Controller Implementation}
Disturbing an weakly damped resonator by applying consecutive momentum kicks inevitably leads to an increase in the average stored energy by the resonator and therefore an increase in its average amplitude. However, since the measurement scheme employed in this work relies on the linear behavior of the resonator, it must remain within the linear operating regime as outlined in Section (\ref{chap:ssnems}). Moreover, suppressing the resonators modal motion and thus its effective temperature might as well lead to other desirable effects such as enhanced frequency stability due to lower heat exchange rates with the thermal bath \cite{zhang2023demonstration}. Hence, an optimal feedback controller (LQR) and state estimator (Kalman-Bucy filter) as summarized in Section~\ref{sec:opt_cntrl} is implemented on the FPGA board.

%The required model includes the three dominant modes visible in the measured spectrum in Figure~\ref{fig:ResSpec}. Which are modelled according to equation (\ref{eqn:MultharmSS}). Additionally, we want to accurately capture the colored measurement noise process. This specifically includes the uninformative resonance peak at \SI{21}{kHz} and the raising measurement noise floor. Such colored measurement noise $\nu$ can be easily included in \eqref{eqn:MultharmSS} by feeding white noise processes $\nu_1$ and $\nu_2$ through a dynamic system of the form
%In total, the stochastic model of the experimental system requires nine states of which six include useful information and the remaining ones model the colored noise processes, i.e., 



==> figures/time_traces/time_traces.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.30100,0.74500,0.93300}%
%
\begin{tikzpicture}

\begin{axis}[%
%width=0.5\textwidth,
%height=0.175\textwidth,
width=1\textwidth,
height=0.35\textwidth,
at={(0in,2.8in)},
%scale only axis,
xmin=0,
xmax=200,
xticklabel=\empty,
ymin=-1e4,
ymax=1e4,
ylabel style={font=\color{white!15!black}},
ylabel={$y$ (\textmu m/s)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]
\addplot [color=mycolor1, forget plot]
  table[x expr=\thisrowno{0}, y expr=\thisrowno{1}*1000000]{figures/time_traces/time_traces-1.tsv};
\addplot [color=red, forget plot]
  table[x expr=\thisrowno{0}, y expr=\thisrowno{1}*1000000]{figures/time_traces/time_traces-2.tsv};
\addplot [color=white!15!black, forget plot]
  table[]{figures/time_traces/time_traces-3.tsv};
\end{axis}

\begin{axis}[%
%width=0.5\textwidth,
%height=0.175\textwidth,
width=1\textwidth,
height=0.35\textwidth,
at={(0in,2.1in)},
%scale only axis,
xmin=0,
xmax=200,
xticklabel=\empty,
ymin=-50,
ymax=50,
ylabel style={font=\color{white!15!black}},
ylabel={$v_1$ (\textmu m/s)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]

\addplot[area legend, draw=none, fill=mycolor2, forget plot]
table[] {figures/time_traces/time_traces-4.tsv}--cycle;
\addplot [color=red, forget plot]
  table[]{figures/time_traces/time_traces-5.tsv};
\addplot [color=white!15!black, forget plot]
  table[]{figures/time_traces/time_traces-6.tsv};
\end{axis}

\begin{axis}[%
%width=0.5\textwidth,
%height=0.175\textwidth,
width=1\textwidth,
height=0.35\textwidth,
at={(0in,1.4in)},
%scale only axis,
xmin=0,
xmax=200,
xticklabel=\empty,
ymin=-50,
ymax=50,
ylabel style={font=\color{white!15!black}},
ylabel={$v_2$ (\textmu m/s)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]

\addplot[area legend, draw=none, fill=mycolor2, forget plot]
table[] {figures/time_traces/time_traces-7.tsv}--cycle;
\addplot [color=red, forget plot]
  table[]{figures/time_traces/time_traces-8.tsv};
\addplot [color=white!15!black, forget plot]
  table[]{figures/time_traces/time_traces-9.tsv};
\end{axis}

\begin{axis}[%
%width=0.5\textwidth,
%height=0.175\textwidth,
width=1\textwidth,
height=0.35\textwidth,
at={(0in,0.7in)},
%scale only axis,
xmin=0,
xmax=200,
xlabel style={font=\color{white!15!black}},
xlabel={time (\textmu s)},
ymin=-50,
ymax=50,
ylabel style={font=\color{white!15!black}},
ylabel={$v_3$ (\textmu m/s)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]

\addplot[area legend, draw=none, fill=mycolor2, forget plot]
table[] {figures/time_traces/time_traces-10.tsv}--cycle;
\addplot [color=red, forget plot]
  table[]{figures/time_traces/time_traces-11.tsv};
\addplot [color=white!15!black, forget plot]
  table[]{figures/time_traces/time_traces-12.tsv};
\addplot [color=white!15!black, forget plot]
  table[]{figures/time_traces/time_traces-13.tsv};
\addplot [color=white!15!black, forget plot]
  table[]{figures/time_traces/time_traces-14.tsv};
\addplot [color=white!15!black, forget plot]
  table[]{figures/time_traces/time_traces-15.tsv};
\end{axis}
\end{tikzpicture}%

==> impulse_results.tex <==
\begin{tikzpicture}
\begin{axis}[
    width = \textwidth,
    height = 0.95\textwidth,
    xlabel style={font=\color{white!15!black}},
    xlabel={input $\Delta v$  (\SI{}{m/s})},
]
\addplot[
color = black,
fill = black,
mark = *,
only marks
] coordinates {
( 338.1, 266.45 )
( 169.1, 143.43 )
( 84.5, 64.80 )
( 42.3, 34.19 )
( 21.1, 9.47 )
};
\addplot[
color = black,
mark = none
] coordinates {
( 0, 0 )
( 350, 279 )
};
\end{axis}
\end{tikzpicture}
